Contrastive Explanations for Model Interpretability

Contrastive explanations clarify why an event occurred in contrast to another. They are more inherently intuitive to humans to both produce and comprehend. We propose a methodology to produce contrastive explanations for classification models by modifying the representation to disregard non-contrastive information, and modifying model behavior to only be based on contrastive reasoning. Our method is based on projecting model representation to a latent space that captures only the features that are useful (to the model) to differentiate two potential decisions. We demonstrate the value of contrastive explanations by analyzing two different scenarios, using both high-level abstract concept attribution and low-level input token/span attribution, on two widely used text classification tasks. Specifically, we produce explanations for answering: for which label, and against which alternative label, is some aspect of the input useful? And which aspects of the input are useful for and against particular decisions? Overall, our findings shed light on the ability of label-contrastive explanations to provide a more accurate and finer-grained interpretability of a model's decision.

==> discarded/0-abstract-discarded.tex <==


% \vspace{-0.5cm}

% Contrastive explanations which elucidate why an event occurred, in contrast to another, have the potential to provide fine-grained interpretability.
% We propose a method based on nullspace projections to produce such explanations in the representation space.
% We demonstrate the value of contrastive explanations in two different scenarios, using high-level conceptual feature attribution for the task, as well as local, highlight feature attributions for individual examples.
% In each setting, adversarial and qualitative evaluations show that explanations which are contrastive are more valuable than conventional explanations \swabha{is that true?}

% Contrastive explanations clarify why an event occurred
% % \yejin{a decision is made as opposed to an event occurred?} 
% \textit{in contrast to} another, and are inherently more intuitive to humans to both produce and comprehend.
% We propose a methodology to produce contrastive explanations for classification models by modifying the representation to disregard non-contrastive information, and modifying model behavior to only be based on contrastive reasoning. 
% % We propose a methodology to produce contrastive explanations in the representation space for predictions in models for text classification.
% % \swabha{Not sure we need a name anymore?}
% Our method is based on projecting model representation to a latent space that 
% % \yejin{`row-space projection' is not the most commonly seen jargon thus should be either explained briefly or at least be accompanied by a citation (or both)} 
% captures only the features that are useful (to the model) to differentiate two potential decisions. 
% We demonstrate the value of contrastive explanations by analyzing two different scenarios, using both high-level abstract concept attribution and low-level input token/span attribution, on two widely used text classification tasks. 
% Specifically, we produce explanations for answering: for which label, \textit{and against which alternative label}, is some aspect of the input useful? And which aspects of the input are useful for and against particular decisions?
% % Specifically, we produce explanations for answering: which label is a feature useful \textit{against}? And which feature is most useful against a label? 
% % \yejin{'for' seems more natural to read than 'against'...} \alon{i mean "against" literally - useful to not predict the label}
% % \swabha{I would rewrite this sentence following Yejin's comment, as well as the part about "feature" - this is not the terminology in the paper (we talk about factors)} \alon{i'm not sure what to do. i don't think factors are good terminology for the abstract...}
% % Specifically, we produce explanations based on which label a given feature is used contrastively against, and which feature is most contrastively useful against a given label.
% % Our experiments show that \name can contrastively distinguish between features for a pair of labels, as well as between labels for a given feature.
% Overall, our findings shed light on the ability of label-contrastive 
% % \swabha{do we use ``label-contrastive'' in the rest of the paper?} 
% explanations to provide more accurate and finer-grained interpretability of a model's decision.
% % \ye{I think there's something more interesting and appealing rather than just a more fine-grained epxlanation.}

% Our experiments with \name show \name's ability to rank the feature space by contrastive power to a given contrast decision, or rank a space of contrastive decisions to a given feature. 
% Our experiments show the usefulness of our methods to derive contrastive explanations, as well as the usefulness of contrastive explanations generally.


% Contrastive explanations clarify why an event occurred in contrast to another. 
% They are more inherently intuitive to humans to both produce and comprehend.
% We propose a methodology to produce contrastive explanations for classification models by modifying the representation to disregard non-contrastive information, and modifying model behavior to only be based on contrastive reasoning. 
% Our method is based on projecting model representation to a latent space that captures only the features that are useful (to the model) to differentiate two potential decisions. 
% We demonstrate the value of contrastive explanations by analyzing two different scenarios, using both high-level abstract concept attribution and low-level input token/span attribution, on two widely used text classification tasks. 
% Specifically, we produce explanations for answering: for which label, \textit{and against which alternative label}, is some aspect of the input useful? And which aspects of the input are useful for and against particular decisions?
% Overall, our findings shed light on the ability of label-contrastive explanations to provide a more accurate and finer-grained interpretability of a model's decision.

% \begin{table*}[]
% \centering
% \resizebox{0.98\linewidth}{!}{%
% \begin{tabular}{cp{10cm}ll} \toprule
%  & Example    & Amnesic Counterfactual & Explained fact/foil                  \\ \midrule
%  (1) & P: An older man with glasses raises his eyebrows in surprise. &   & \multirow{2}{*}{\textit{contradiction} rather than \textit{entailment}}   \\
%  & H: The man \hl{has no} glasses. & The man \_\_\_ glasses. &  \\ \midrule
%  (2) & P: An older man with glasses raises his eyebrows in surprise. &       & \multirow{2}{*}{\textit{entailment} rather than \textit{contradiction}} \\
%  & H: The man \hl{wears} glasses. & The man \_\_\_ glasses. &  \\ \midrule
%  (3) & P: An older man with glasses raises his eyebrows in surprise. &       & \multirow{2}{*}{\textit{entailment} rather than \textit{neutral}} \\
%  & H: The man wears \hl{glasses}. & The man wears \_\_\_. &  \\
%   \bottomrule
% \end{tabular}}
% \caption{Example text in \textit{natural language inference}, from data by  \citet{DBLP:conf/iclr/KaushikHL20}, to demonstrate contrastive explanations. Depending on which decision is being explained (\textit{fact}), \textit{and depending on which decision it is explained \textbf{against}}, the explanation may change, or be understood differently. \ye{I would make the premise on top, and then just show the hypotheses with some arrows.
% e.g.
% P: ...
% sep line
% -> H: ...
% sep line
% -> H: ...
% ...}}
% \label{tab:intro-example}
% \end{table*}

% \begin{table*}[]
% \centering
% \ra{1.15}
% \resizebox{0.98\linewidth}{!}{%
% \begin{tabular}{cp{6cm}lll} \toprule
%  & Example    & Decision & Amnesic Counterfactual  & Explained decision                  \\ \midrule
%   & P: An older man with glasses raises his eyebrows in surprise. &   & \\ \midrule
%  (1) & H: The man \hl{has no} glasses. & \textit{contradiction} & The man \_\_\_ glasses. &  \textit{contradiction} rather than \textit{entailment} \\ 
%  (2) & H: The man \hl{wears} glasses.& \textit{entailment} & The man \_\_\_ glasses.  & \textit{entailment} rather than \textit{contradiction} \\ 
%  (3) & H: The man wears \hl{glasses}. &\textit{entailment} & The man wears \_\_\_. &  \textit{entailment} rather than \textit{neutral} \\
%   \bottomrule
% \end{tabular}}
% \caption{Example text in \textit{natural language inference}, from data by  \citet{DBLP:conf/iclr/KaushikHL20}, to demonstrate contrastive explanations. Depending on which decision is being explained (\textit{fact}), \textit{and depending on which decision it is explained \textbf{against}}, the explanation may change, or be understood differently. 
% }
% \label{tab:intro-example}
% \end{table*}

==> discarded/7-discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}

Given the relative novelty of contrastive explanations in NLP and ML research, there remain several open questions in this topic, which are potential future directions of research.
% We list a few of them below.

\paragraph{Evaluating explanations.} Evaluation of explanations in neural NLP models is a difficult and ongoing research area. 
While the mathematical interpretation of our methodology is sound, some questions on evaluation remain.
% what should foils satisfy in order to be more intuitive to humans (and how can we measure the degree of intuitiveness)? 
How can we choose foils such that explanations are more comprehensible to humans?
Similarly, what should causal factors satisfy, in terms of their \textit{social attribution} \cite{jacovi2020aligning}?
% \swabha{very vague...remove or add more detail.}
Our work provides sanity-check evaluations based on data staining. 
Additionally, our experimental results align with prior intuition on well-researched models and tasks. 
% We theorize that psychological or philosophical research, as well as user experimentation, will be useful in answering additional questions on utility of contrastive explanations. \swabha{what psychological research?}
% Human evaluations might be used to evaluate the quality of contrastive explanations; however, most human evaluation via crowdsourcing platforms tends to be noisy \cite{ipeirotis2010quality}. \alon{i don't agree witht his sentence - i generally don't agree with using human evaluation in explainability, or at least, i think it's very problematic and nontrivial to think about its potential issues}

\paragraph{Types of interventions.} 
Our amnesic interventions, e.g., masking highlights, and latent space concept removal, generate counterfactual representation for behavioral analysis. 
However, amnesic counterfactuals do not provide a complete picture of how humans comprehend decision processes: the information communicated in the explanation is contextual in the type of intervention applied. 
Currently, literature is limited for the 
% exact attributes and 
trade-offs between various types of interventions (and types of counterfactuals) in explanation. 
Additional research in this area may answer what exactly do amnesic counterfactuals do and do not communicate, and how to categorize classes of possible counterfactuals by their utility. 
% We also provide a non-amnesic manually created counterfactual setting (\S\ref{sec:e-snli}).

% \paragraph{Limitations of the interventions.} Two of the interventions in this work---amnesic probing and the contrastive projection (as the intervention itself; \S\ref{ssec:contrastive-intervention})---focus on the final classification layer in the model. In the case of amnesic probing, it is theoretically possible that this information is utilized for some role in the reasoning process, and then ``forgotten'', prior to the final layer. We theorize that this is \textit{impossible}, i.e. that  in the case of the contrastive projection this effect cannot happen, but we leave proof of such to future work.
% \swabha{given that we don't know if this really happens I would skip this paragraph.}
% In this case, the intervention will \textit{not} discover the causal role of the factor in the decision process, since we intervene after this role is finished.

% Future work?
% 1. Backprop through the contrastive layer. Possible applications: Reducing the highlight search space with (contrastive) gradient saliency maps
% 2. More research on different types of counterfactuals/interventions and bifactuals with contrastive influence functions
% 3. Can we use this contrastive analysis of models trained on human data to analyze the contrastive nature of human annotation? (for instance NLI)

\section{Conclusion}
\label{sec:conclusion}

We proposed a framework for producing contrastive explanations in text classification. 
Our framework is based on selection from a pre-defined space of candidate factors and model decisions.
We presented a behavioral analysis where results were measured as change in model behavior following an intervention. 
We propose a theoretical (mathematical) modification of model behavior into a contrastive reasoning process, which allows the behavioral change to be interpreted in the context of a particular alternative decision. 
% \swabha{i'm not able to understand this sentence}
Our framework is flexible and generalizable, as is demonstrated via our experiments with two text classification tasks on BIOS and MultiNLI.
% tasks, which demonstrates its flexibility and utility, and derives useful conclusions on typical models trained on those tasks. 
Overall, we observe, via quantitative and qualitative evaluations, that a contrastive context to explanations makes them easier to understand, and allows finer-grained communication of aspects of model behavior. 
% Explanations are inherently contrastive, therefore formulating them explicitly as such allows more rigorous explainability of models. 
% \alon{last paragraph can be deleted?}


